UniHeap: Managing Persistent Objects Across Managed Runtimes for Non-Volatile Memory

Byte-addressable, non-volatile memory (NVM) is emerging as a promising technology. To facilitate its wide adoption, employing NVM in managed runtimes like JVM has proven to be an effective approach (i.e., managed NVM). However, such an approach is runtime specific, which lacks a generic abstraction across different managed languages. Similar to the well-known filesystem primitives that allow diverse programs to access same files via the block I/O interface, managed NVM deserves the same system-wide property for persistent objects across managed runtimes with low overhead. In this paper, we present UniHeap, a new NVM framework for managing persistent objects. It proposes a unified persistent object model that supports various managed languages, and manages NVM within a shared heap that enables cross-language persistent object sharing. UniHeap reduces the object persistence overhead by managing the shared heap in a log-structured manner and coalescing object updates during the garbage collection. We implement UniHeap as a generic framework and extend it to different managed runtimes that include HotSpot JVM, cPython, and JavaScript engine SpiderMonkey. We evaluate UniHeap with a variety of applications, such as key-value store and transactional database. Our evaluation shows that UniHeap significantly outperforms state-of-the-art object sharing approaches, while introducing negligible overhead to the managed runtimes.

==> ack.tex <==
\section*{Acknowledgments}
We would like to thank the anonymous reviewers and shepherd Jonathan Balkind for their
helpful comments and feedback. This work was partially supported by the NSF grant CNS-1850317, CCF-1919044, 
and CNS-1763658. 




==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%In this paper, 
We present \pname{}, a unified persistent object management 
for different managed runtimes. \pname{} is driven by the trend that managed runtime 
would be the new abstraction to manage NVM. 
%However, existing approaches are either 
%runtime specific or lacking support of data persistence. 
%As the system-wide shared resource, non-volatile 
%emories deserve the property of persistent object sharing across diverse 
%anaged runtimes. 
%first NVM programming framework that 
\pname{} provides a more generic NVM programming framework by enabling 
persistent object sharing across various managed runtimes. %and efficient data persistence. 


==> implt.tex <==
\vspace{-2ex}
\section{\pname{} Implementation}
\label{sec:implt}
In this section, we describe the \pname{} implementation details. 
We will first discuss the implementation of the main framework. 
And then, we will 
present the module implementation for each individual managed runtime, 
including HotSpot JVM, cPython, and SpiderMonkey. 

\noindent
\textbf{Main Framework Implementation.}
We implement \pname{} system prototype with 9,163 lines of C programming code. 
The \pname{} framework is implemented as a shared library, 
%and has 4,092 lines of C code, 
including \pname{} interface and GC for the log region. 
As for the shared NVM heap, \pname{} uses the memory-mapped interface with 
Direct Access (DAX)~\cite{Xu-fast16} enabled for fast access to the NVM device. 
Each runtime module will dynamically load this shared library at the runtime initialization.  
%and then, the runtime will resolve the symbols of \pname{} interfaces in the shared library. 
The \pname{} server proxy implementation has 5,732 lines of C code, including 
process communication and GC. 
%The HotspotJVM module and CPython 
%module have 1,206 and 568 lines of codes respectively. 
%In this following, 
%we describe the implementation details of Hotspot JVM, CPython, and SpderMonkey, 
%respectively. 
%\pname{} requires a DAX-aware file system (e.g., Ext4-DAX) to memory map the heap file into server and runtime address space.

%There is a server process managing all non-volatile heaps. Each \pname{} module creates a \pname{} thread to communicate with the server process via UNIX domain socket. \pname{} minimize the inter-process communication during runtime execution. In particular, the \pname{} module only communicate with the \pname{} server during runtime initialization and object garbage collection. For the runtime initialization, \pname{} module communicate with the server to create the shared memory, load the shared heap, and initialize other system state. On the other side, once \pname{} start to GC, all runtime must report their \textit{vroot} to the \pname{} server process. Moreover, \pname{} also need to coordinate with other runtimes to stop the world through this communication channel.
%We also provide a \textsc{MkHeap} tool to format a normal file into our heap layout. \pname{} server leverages existing \emph{DAX} feature provided by the commidity file system (i.e., Ext4) to memory mapping the heap file into \pname{} server address space. Other runtime which loaded the heap also memory mapped the heap file into their address space in the same virtual addresses.

\noindent
\textbf{Hotspot JVM Implementation.}
We modify a few OpenJDK8u212-b03-0 components to support \pname{}. 
We modify the Hotspot template interpreter to implement our transaction mechanism. 
We add hook functions in the bytecodes for object field accesses (i.e., \emph{putfield} 
and \emph{getfield}), and array element access (e.g., \emph{arrayload} and \emph{arraystore}).
We also modify the parallel scavenge GC to support our GC for persistent objects. 
Specifically, we add the remembered sets~\cite{wwwgc} support in the GC procedure. 
%During young GC procedure, 
After the GC copies all objects to the \emph{from} region, 
the runtime module reports all the remaining live objects as \emph{vroots} to \pname{}.  
%In addition, we also extend the card table for the tenured region to track the references 
%from JVM runtime to our persistent object.

\noindent
\textbf{cPython Implementation}
For the Python runtime, we use the open-source cPython 2.7.15.  
%We modify the bytecodes of cPython to enable the read and write to persistent objects. 
We add the hook functions in the corresponding bytecodes for object accesses, such as 
\emph{LIST\_APPEND}, \emph{LOAD\_LOCALS}, \emph{LOAD\_ATTR}, \emph{STORE\_LOCAL}, 
and \emph{STORE\_GLOBAL}. 
%Since Python is a dynamic language, we also add hook
%how we handle molding from class descriptions to a Plass from it, 
%meaning we must also hook bytecode \emph{BUILD\_CLASS}. 
%Obtaining vroots is a bit more tricky due to 
Since cPython uses a reference counter-based GC rather than a tracing-based one, 
special effort is required to obtain the object references. 
In cPython, a module is used to implement a generational GC 
on top of the reference counter based GC, in which object deallocation happens when its 
reference count drops to zero. Therefore, we can obtain \emph{vroots} by tracking 
the object references from their allocation to deallocation. 
%it is challenging to obtain the \emph{vroots}.
%with an optional module to implement a generational garbage collector on top of it, 

%Since the generational GC also uses a (modified) reference counting scheme, 
%we can remember vroots by simply tracking them from allocation to deletion, 
%which we know occurs when the reference count in the \emph{PyObject} struct 
%hits 0 in \emph{Py\_DECREF}.


\begin{comment}
\begin{itemize}
	\item template interpreter
	\item generational heap space
	\item parallel scavenge garbage collector
	\item uniheap framework module
\end{itemize}
\end{comment}

%\subsection{JavaScrip SpiderMonkey Implementation}
\noindent
\textbf{JavaScript Implementation.}
Similar to HotSpot and cPython, \pname{} adds hook functions to the relevant bytecodes for object accesses 
in SpiderMonkey with version 52. They include 
%The relevant bytecodes in Spidermonkey to hook are, once again, those to do with reading from 
%or writing to possibly persistent objects
\emph{JSOP\_GETLOCAL}, \emph{JSOP\_SETLOCAL}, \emph{JSOP\_GETNAME}, \emph{JSOP\_SETNAME}, and others. 
%\emph{JSOP\_STRICTSETNAME}, and so on. %\emph{JSOP\_GETINTRINSIC}, and so on. %\emph{JSOP\_SETINTRINSIC}, and so on. 
The GC of SpiderMonkey is similar to that of HotSpot JVM. Their major difference is that 
the marking phase in SpiderMonkey occurs incrementally. But the way of tracking \emph{vroots} 
in SpierMonkey is similar to that of HotSpot JVM. The SpiderMonkey runtime module reports 
its \emph{vroots} when copying them to a new heap during the GC. 
%Instead of using a card table, 
%SpiderMonkey utilizes a \textit{store buffer} for its cross-generational edges, we leverage 
%this buffer to obtain \emph{vroots}. 
%Moreover, SpiderMonkey provides 
%a function named \emph{JS::PersistentRooted<T>} to set a root object from which others can stem,  
%we also hook this function to obtain the \emph{vroots}.


==> macros.tex <==

\newcommand{\Eg}{{\em E.g.}, }
\newcommand{\eg}{{\em e.g.}, }
\newcommand{\ie}{{\em i.e.}, }
\newcommand{\etal}{{\em et al.}}
%\newcommand{\pname}[1]{{{{FlatFlash}}}{#1}}
\newcommand{\pname}[1]{{{\textsc{UniHeap}}}{#1}}
%\newcommand{\palg}[1]{{{\textsc{Havz}}}{#1}}
\newcommand{\palg}[1]{{{adaptive}}{#1}}


\newcommand{\website}[1]{{\tt #1}}
\newcommand{\program}[1]{{\tt #1}}
\newcommand{\benchmark}[1]{{\it #1}}
\newcommand{\fixme}[1]{{\textcolor{red}{\textit{#1}}}}

\newcommand*\circled[2]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill=black,inner sep=1pt] (char) {\textcolor{#1}{{\footnotesize #2}}};}}

\ifx\figurename\undefined \def\figurename{Figure}\fi
\renewcommand{\figurename}{Figure}
\renewcommand{\paragraph}[1]{\textbf{#1}~~}
\newcommand{\figline}{{\vspace*{.05in}\hline}}

\newcommand{\Sect}[1]{$\S$~\ref{#1}}
\newcommand{\Fig}[1]{Figure~\ref{#1}}
\newcommand{\Tbl}[1]{Table~\ref{#1}}
\newcommand{\Equ}[1]{Equation~\ref{#1}}
\newcommand{\Apx}[1]{Appendix~\ref{#1}}

\newcommand{\specialcell}[2][c]{\begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\newcommand{\niparagraph}[1]{\vspace{3pt}\noindent\textbf{#1}}

\usepackage[labelfont=bf, font={}]{caption}



% checkmark and xmark in the pifont package
%\newcommand{\cmark}{\ding{51}}
%\newcommand{\xmark}{\ding{55}}



==> motivation.tex <==
\section{Background and Motivation}
\label{sec:motivation}
%Technical challenges for managed language in persistent memory era:
%
%\begin{itemize}
%	\item Managed languages require data persistence and sharing support for objects.
%	\item Current object persistence solution has to serialized/deserialized the object first.
%	\item Current object approach has to marshall/demarshall the object first.
%	\item File system \& database system are heavy-weight system abstractions to persist the data.
%\end{itemize}

\subsection{Byte-Addressable NVM}
\label{subsec:nvm}
%NVM is emerging as a revolutionary technology for computer systems. 
%Recently, Intel released its first NVM device~\cite{intel:optane}, marking that the byte-addressable 
%NVM has become realizable. 
Compared with conventional DRAM, NVM provides much higher density, allowing 
it to have larger storage capacity. 
%However, the speed of NVM is slower than DRAM~\cite{Qureshi-isca09,3DXPoint}. 
%Therefore, hybrid memory consisted of both DRAM and NVM, has been proposed as a practical 
%solution. It allows applications to allocate data to either DRAM or NVM, depending on 
%the performance and data durability requirements from applications. 
NVM provides data durability, which allows it to be used as persistent 
storage. However, it requires memory persistency to ensure the crash 
consistency~\cite{Pelley-isca14, mnemosyne, Kolli-asplos16, whisper}. 

Ensuring memory persistency is challenging with modern memory 
hierarchy, as many levels of volatile cache (e.g., volatile processor cache and DRAM) exist 
between the processor and NVM.  
%care must be taken to ensure that a processor store to NVM propagates
%its value to NVM, rather than leaving it the cache hierarchy.
%from the processor becomes
%persistent. In other words, we need to ensure that the stored value
%is propagated to
%NVM, rather than being hidden by the cache hierarchy.
With commodity out-of-order processors, the order in which stores 
are made persistent depends on the order they are evicted from the cache. % hierarchy.  
%To ensure the data consistency, specific instructions such as \emph{clflush} and \emph{mfence} 
%are used. 
%To ensure that  store values reach  NVM deterministically,
%they must be written back from the cache
%via explicit instructions. Further, to guarantee a distinct ordering,
%fences must be inserted.
%%inserted to guarantee a distinct ordering.
%%we need special st} instructions.
%%must be performed to ensure a store reaches NVRAM.
Therefore, explicit instructions have to be used.  
For instance, x86-64 processors have the \emph{clwb}
instruction~\cite{intel:clwb} to write back a cache line from the processor cache 
to NVM, %without flushing it from the cache. 
%And multiple such cache line
%writebacks are allowed to be internally reordered by the hardware
%unless fences are placed in the code. 
and storage fence instruction (\emph{sfence}) to 
guarantee that a \emph{clwb} instruction completes.  
%one needs to
%add the x86-64 storage fence (\emph{sfence}) instruction.
However, %requiring end users to deal with the memory persistency 
this will inevitably 
increase the burden of software development and the complexity of NVM 
management. %This drives the recent development of NVM frameworks. 

\subsection{NVM Management and Programming}
\label{subsec:nvmsys}
To facilitate the use of NVM, both industry and academic community have developed 
high-level libraries and system frameworks. They 
%Intel has developed a high-level 
%library, named Persistent Memory Development Kit (PMDK), which 
enable programmers to develop durable applications on top of NVM, without 
dealing with the low-level primitives~\cite{pmem:PMDK, nv_heaps, mnemosyne, 
microsoft_nvm, hp_atlas, nv_threads, whisper, nvl-c, Xu-fast16, Rao-eurosys14}.
%However, PMDK requires programmers to either use demarcated failure-atomic 
%regions or explicitly specify data structures that need to be persisted.
%The academic community also developed many frameworks for 
%NVM~\cite{nv_heaps, mnemosyne, microsoft_nvm, hp_atlas, nv_threads, whisper, nvl-c, 
%Xu-fast16, Rao-eurosys14}. 
%Although they propose different ways of organizing data structures in NVM, 
Their abstraction for developers is similar, 
which requires developers to specify the durable data structures and failure-atomic 
regions for ensuring the crash-safety. 

Recently researchers proposed to leverage managed runtimes like JVM to 
manage NVM~\cite{espresso, Shull-pldi19, nvmgc:pldi2018, panthera:pldi19}. 
Such an approach is promising to simplify the NVM programming. 
For instance, %Espresso~\cite{espresso} enables persistent object support for NVM in JVM; 
AutoPersist~\cite{Shull-pldi19} only requires 
%further simplifies the NVM programming by only requiring 
developers to explicitly specify the durable root objects, the managed runtime will 
automatically persist the reachable objects based on the 
reachability analysis in JVM. 
%Write Rationing~\cite{mckinley_nvm_gc} exploits the GC procedure 
%in JVM to optimize the object placement to reduce the write traffic to NVM. 
%which significantly extends the NVM lifetime. 
As a majority of applications today are developed with managed languages such as 
Java and Python~\cite{popular-language, managed-language}, 
these prior studies make us believe 
the runtime-based approach is becoming a pervasive and practical solution for managing NVM.    

%\subsection{Why A Generic NVM Framework}
%\subsection{Why Managing Persistent Objects Across Runtimes}
%\subsection{Why Object Sharing Across Runtimes}
\subsection{Object Management Across Runtimes}
\label{subsec:why}
The current approach of managing NVM is runtime specific. It lacks an important property: 
persistent object management across managed 
runtimes. Similar to the system-wide shared persistent storage whose management 
software -- file systems -- enable the data sharing across different programs 
with the \textit{file} abstraction, the runtime-managed NVM 
framework is desirable to enable the data sharing with the \textit{persistent object} 
abstraction, such that the objects created by one managed runtime can be 
easily accessed by another one.   

This property will benefit many real-world application cases, such as web 
services~\cite{xmem:pldi2008, trufflevm:dls2015} and data analytics~\cite{skyway, hive:vldb2009, spark}. In these applications, 
multiple runtime instances access shared data source for further analytics, 
and different instance may fulfill different functions~\cite{multiprogram}.  
For example, (1) a Java program persists its objects in NVM and allows other programs written 
in a different language such as Python to access them directly (e.g., web services); 
(2) a Java program and Python program concurrently access shared persistent objects (e.g., 
shared libraries); or (3) multiple Java programs concurrently access a persistent object (e.g., 
data analytics).  

 
To achieve the same property, existing managed runtimes persist 
objects to file systems or database in NVM. 
However, they suffer from significant software overheads~\cite{espresso}. 
Typical examples include Java Persistence API (JPA) that uses transactional 
APIs to persist data~\cite{java-persistence}, and Persistent Collection for 
Java (PCJ)~\cite{PCJ} that manages Java objects in NVM.  
Both methods have the data transformation procedure, which introduces dramatic 
performance overhead. 
%In this paper, we aim to develop a lightweight mechanism for enabling object persistence 
%and sharing across managed runtimes. 
%with minimal data persistence overhead.  
%Similar to the filesystem abstraction 
%for the persistent storage, managed NVM deserves the data sharing as shared resources, 
%which enables different managed languages to access the persistent objects efficiently. 


%The Storage Networking Industry Association (SNIA) has been
%working to standardize the interactions with NVM. It has created a
%low-level programming model~\cite{snia:nvm_model} meant to be followed by device
%driver programmers and low-level library designers. In addition, an open source
%project led by Intel has been created to provide application developers a
%high-level toolset that
%is compliant with SNIA's device-level model. This
%project has resulted in the development of the Persistent Memory Development Kit
%(PMDK)~\cite{pmem:PMDK}, a collection of libraries in C/C++ and Java
%that a
%developer can use to build durable applications on top of NVM.
%
%PMDK requires that programmers explicitly label all the durable data
%in their code with pragmas. As an alternative, PMDK also contains a few
%library data structures, such as a durable array and hashmap, with the necessary
%persistent pragmas already built into the library.
%
%For persistently storing data, PMDK requires the
%programmer to
%either explicitly persist stores, or use demarcated
%failure-atomic regions. Failure-atomic regions
%enable  many stores to persistent memory to appear to
%be persisted atomically.
%Recently, PMDK has also introduced C++ templates that allow some
%operations to be persistent without explicit user markings.

%Academia Second
%In addition to the industrial efforts, academia has also proposed
%several
%frameworks for NVM~\cite{espresso, nv_heaps, mnemosyne, microsoft_nvm,
%hp_atlas, nv_threads, whisper, nvl-c}. The
%level of support provided by these frameworks varies. At most, they provide a
%similar level of abstraction as PMDK, with the user having to specify all
%durable objects and also providing some minimal failure-atomic region support.
%



==> related.tex <==
\section{Related Work}
\label{sec:related}
%\niparagraph{Non-volatile Memory Management.}

\noindent
\textbf{Programming Frameworks for NVM.}
To facilitate the use of NVM, many NVM frameworks have been proposed~\cite{espresso, 
nv_heaps, mnemosyne, microsoft_nvm, hp_atlas, nv_threads, whisper, nvl-c, 
language_level_persistence, pmem:PMDK, larus_epfl}. All of these works require the programmer 
to explicitly specify the data structures that should reside in NVM.  
This limitation requires significant effort from programmers, potentially causing correctness 
and performance bugs in NVM programs. 
%In other words, these NVM frameworks are still not easy to use. 
Recent studies such as AutoPersist~\cite{Shull-pldi19} and 
Espresso~\cite{Wu-asplos18} proposed to exploit the managed runtime to manage NVM, which simplifies 
the NVM programming. However, these runtime-based solutions are mainly developed based on JVM, 
which cannot work as a generic programming framework. Our work \pname{} extends this thread of 
research to other managed languages such as Python and JavaScript, while enabling efficient  
persistent object sharing across different runtimes.        
%and sometimes even apply 
%various crash-consistency techniques such as logging and shadow paging to ensure memory persistency. 
%While most existing frameworks are 
%written in C or C++, Wu et al.~\cite{espresso} proposed to integrate NVM into Java runtime. Similar to 
%previous studies, the user has to explicitly identify all non-volatile allocations, and perform the persist operations necessary for crash consistency. 
%Section~\ref{sec:eval} compares \pname{} and Espresso. 
%\pname{} also provides APIs for developers to support both manual data persistence and automatic data 
%persistence. 
%Atomic Region Support

\begin{table}[t]
    \footnotesize
        \caption{Number of incurred \emph{mfence} operations.}
    \label{tab:mfence}
        \vspace{-3ex}
    \centering
    \begin{tabular}{|l|l|l|}
                \Xhline{0.9pt}
                \textbf{Benchmarks}  & \textbf{AutoPersist} & \textbf{\pname{}}\\
                \Xhline{0.9pt}
                Workload A & 1798 & 18 \\
                Workload B & 398 & 4 \\
                Workload C & 0 & 0 \\
                Workload D & 331 & 6 \\
                Workload F & 1898 & 22 \\
                \Xhline{0.9pt}
    \end{tabular}
        \vspace{-4ex}
\end{table}



\noindent
\textbf{Reduce Memory Persistency Overhead.}
NVM requires memory persistency operations to ensure crash consistency~\cite{pelly_memory_persistency, mnemosyne, Kolli-asplos16, whisper}. However, ensuring memory persistency with modern memory hierarchies 
is challenging. To alleviate memory persistency overhead, 
prior studies proposed both software~\cite{harris_memory_persistent,wenisch_2,wenisch_sfr,mnemosyne, 
nvlogging_jian} and hardware~\cite{atom_hardware_intel, hardware_rice_tx,proteus_ncstate} techniques 
to reduce the overhead of logging in atomic regions and transactions.
\pname{} manages persistent objects in a log-structured manner, which avoids double writes and 
significantly reduce the logging overhead.

\noindent
\textbf{Persistent Object Sharing.}
As system-wide shared resources like persistent storage, NVM deserves efficient data sharing 
across different managed runtimes. JVM has developed 
persistence layers to persist objects to file systems or database, including 
Java Persistence API (JPA)~\cite{java-persistence} and Java Data Objects (JDO)~\cite{jdo}. 
However, they still suffer from significant object serialization/deserialization overhead. 
%The protocols such as Thrift~\cite{thrift} and Protocol Buffers~\cite{protocolbuffers} 
%developed by the industry have similar performance overhead. 
The most efficient approach for 
enabling cross-language communication is the shared memory~\cite{Wegiel-oopsla10}. 
However, the existing study did not support NVM and data persistence. 
To the best of our knowledge, \pname{} is the 
first work that enables persistent object sharing across various managed runtimes. 

 

%Forwarding pointers and write barriers are used in concurrent and generational garbage collectors~\cite{pizlo_gc,metronome,shenandoah,g1gc,azul_c4}. 
%To the best of our knowledge, this the first time that such runtime techniques have been
%applied to help create
%crash-consistent applications in NVM. This use case is different from GC,
%since the behavior is dictated by static user markers
%instead of the temporal behavior of GC.
%%and hence can be
%%optimized.
%%accordingly.
%However, \pname{}'s forwarding pointers and barriers can
%be shared with GC when used in conjunction with advanced GC
%implementations.
%Analysis techniques have been proposed to anticipate long living
%objects~\cite{blackburn_pretenure}, to
%prevent wearout~\cite{mckinley_nvm_gc}, and to predict when object resources can be
%reclaimed~\cite{guyer_gc,xu_gc}. We expect to further improve \pname{}
%with such techniques.
%
%
%%performance in the future by leveraging such techniques already present in current literature.
%
%Many persistent programming languages~\cite{ps_algo, pm3, persistent_oberon,
%orthogonal_persistence_java, e_language, texas_language} and
%implementations~\cite{pjama, pevm_java, blackburn_persistent_java} were
%proposed before the introduction of byte-addressable NVM. These languages 
%focus on attaining the {orthogonal persistency} defined
%by Atkinson and Morrison~\cite{seminal_orthogonal_persistence}, where the
%persistency of an application is transparent to its design.
%%
%The persistency model in \pname{} is different from that, as 
%it does not seek to attain complete orthogonal persistency.
%Furthermore, previous papers on orthogonal persistency proposed approaches to
%optimize the two-level storage model with orders of magnitude performance differences, 
%whereas \pname{} mainly targets byte-addressable NVM.
%
%%Persistency Models
%
%Previous papers have proposed many persistency models~\cite{pelly_memory_persistency, scott_linearizability,
%language_level_persistence, boehm_persistence_model, mutlu_loose_ordering, wenisch_sfr}. 
%They define how
%stores to NVM can be reordered both in software and hardware.
%%\pname{}'s persistency model is described in
%%Section~\ref{sec:model:persistency}.
%Currently,  \pname{} uses sequential persistency outside of failure-atomic regions and
%epoch persistency inside failure-atomic regions. 
%%However, more relaxed persistency
%%models can leverage our runtime reachability analysis.
%

